Gender and Emotion Recognition from Implicit User Behavior Signals

This work explores the utility of implicit behavioral cues, namely, Electroencephalogram (EEG) signals and eye movements for gender recognition (GR) and emotion recognition (ER) from psychophysical behavior. Specifically, the examined cues are acquired via low-cost, off-the-shelf sensors. 28 users (14 male) recognized emotions from unoccluded (no mask) and partially occluded (eye or mouth masked) emotive faces; their EEG responses contained gender-specific differences, while their eye movements were characteristic of the perceived facial emotions. Experimental results reveal that (a) reliable GR and ER is achievable with EEG and eye features, (b) differential cognitive processing of negative emotions is observed for females and (c) eye gaze-based gender differences manifest under partial face occlusion, as typified by the eye and mouth mask conditions.

==> Discussion_backup.tex <==
\section{Discussion \& Conclusion}\label{Con}
%ICMI_discussion and con.
A critical requirement of today's ubiquitous computing devices is to sense user intention, emotion and cognition from multimodal cues, and devise effective interactions to optimize users' individual and social behaviors. Affective computing (AC), whose objective is to empower devices to interact naturally and empathetically with users, plays a crucial role here. Apart from inferring user emotions, it would also be beneficial for AC systems to predict \emph{soft biometrics} such as user \emph{age} and \emph{gender} for effective interaction~\cite{Rukavina16}. There is also a strong need to develop sensing mechanisms that respect user privacy concerns~\cite{Reynolds04}, and eye-movements and EEG signals represent \emph{privacy preserving implicit behaviors} which enable inference of user traits even as the user identity remains hidden. 

The primary objective of this study is to explore the utility of eye movements and EEG for \emph{user gender} prediction. We designed a study where these implicit user behaviors were recorded as 28 users (14 male) recognized facial emotions; since eye movements are known to be characteristic of the perceived facial emotion~\cite{schurgin,subramanian2011can}, our study design additionally enabled recognition of the \emph{facial} (stimulus) \emph{valence}. Crucially, our study employs lightweight and inexpensive sensors for inference, as against bulky and intrusive lab sensors which are typically used in user-centered analyses but significantly constrain user behavior. Also, to examine user efficacy for FER under occlusions, we presented both unoccluded (high and low-intensity), and occluded (with the eye or mouth region masked) emotive faces to users.

The fact that gender differences exist in visual emotional processing is demonstrated at multiple levels via our experiments. In terms of \emph{explicit} user responses, female users are found to quickly and accurately perform FER on unoccluded faces, especially for negative valence emotions (Section~\ref{DA}). Likewise, females also achieve higher recognition of negative emotions with mouth-masked faces. Subsequent examination of \emph{implicit} cues revealed interesting correlations; examination of eye fixation distributions showed that females fixated more around the eyes than males irrespective of the stimulus condition, and female fixation durations were significantly higher in the mouth-mask condition. This observation is consistent with prior studies~\cite{wells2016identification}, and the proposition that females primarily look at the eyes for emotional cues.     

Analysis of EEG ERPs also conveyed some interesting patterns. In response to unoccluded emotive faces, stronger N100 and P300 peaks are noted in female ERPs for negative emotions, as well as a stronger N400 peak for strongly negative faces. This suggests a differential cognitive processing of negative vs positive emotions by females, which results in their enhanced sensitivity towards negative emotions. Likewise, lower male N400 latencies are generally noted at the O2 electrode for positive emotions. Stronger N100 and P300 female ERPs are also noted with negative mouth-masked faces, suggesting that negative emotions are processed rapidly by women, and do not  necessarily entail selective attention to emotional cues. 	 	  
  
That implicit and differential behaviors such as eye fixation distributions and EEG ERPs can be isolated using low-cost sensors affirms that our experimental design can effectively capture emotion and gender-specific information. Greater female sensitivity to negative emotions can be attributed to several factors like social structure, environment and evolution, way of living and social stereotypes\cite{deng2016gender}. While we did not seek to expressly induce emotions in viewers through facial imagery, facial expressions are known to induce emotions in the viewer~\cite{Siedlecka19}, and examination of users' emotional behavior enables prediction of both the {user gender} and {stimulus valence}.

%Though our current task does not involve explicit invoking of emotions through stimuli i.e the task of emotional experience where gender differences were found in emotional experience of negative emotions. We have encountered a qualitative existence of gender differences in recognition(or analysis) of emotions similar to \cite{deng2016gender}. 
SUMMARIZE EXPERIMENTS & RESULTS

%A near perfect GR with EEG (peak AUC of 0.93), eye features (peak AUC of 0.97) and their fusion (peak AUC of 0.97), as well as valence recognition (peak AUC of 0.99 with eye data) is achieved using the deep learning framework and AdaBoost algorithm respectively. The use of minimally intrusive and low-cost devices for studying user behavior makes our findings ecologically valid, and enhances the possibility of large-scale user profiling. Emotion and gender recognition experiments with EEG and eye-based features, as well as their combination revealed that optimal recognition of emotional valence is achieved with eye-based features, while best GR performance is achieved with EEG irrespective of the machine learning method used. Though the best GR with emotion-specific features is observed with \textit{happy} in case of EEG, the negative emotions(anger and sad) perform close to it. Also the gaze features confirm that the best GR is achieved with negative emotions which is consistent with our observations from table-\ref{GenResults}. EEG features generally outperform eye-based features for the purpose of GR. The fusion of EEG and gaze features has not significantly contributed to the performance however it is to be noted that in case of eyemask morphs, the performance is higher than that of either of the modalities. Similarly for emotion-wise GR, the mouthmask morphs outperformed the best of the modalities.

The gender differences in facial emotion perception have been exploited to achieve better performance in terms of ER and GR performance, especially considering that implicit user behavioral cues are acquired with low cost sensors, and also consistent with prior observations. Lithari \etal~\cite{Lithari2010} noted amplitude and phase-related differences for positive and negative emotions in males and females, and some of these findings are mirrored in our ERP analyses. Several eye tracking works (\eg, see~\cite{halljudith}) have noted enhanced female sensitivity for negative emotions, while other neural studies~\cite{Mclure04} have noted that gender differences in emotion processing are best encoded by the frontal and occipital brain lobes. As strong GR (max AUC = 0.97) is achievable with the considered features. This does not involve manual intervention in preprocessing the data for eyeblinks, muscle movements and electrical interference. Thus suggesting a real-time utilization of such methods of user profiling using low-cost devices with fewer electrodes and low sampling frequency(as demonstrated from our spatial analyses results and downsampling to 32Hz for deep learning model). \textcolor{blue}{Better performance of the deep learning model suggests that EEG information in its raw form is reliable to the task at hand when compared to using dimensionality reduction techniques such as PCA coupled with conventional methods}. This also offers a chance to further exploit the low-cost devices for more complex BCI applications that could make the BCIs affordable to general population and more importantly, the people with disabilities.
%using deep learning making the BCIs affordable to general population and more importantly, the people with disabilities.


The larger aim of this work is to predict user demographics via implicit and anonymous behavioral cues so as to implement intelligent advertising, recommendation systems and mental health monitoring systems(for disorders like Alexithymia).Some of the applications are described here. A recommendation system could be built by evaluating user engagement in advertisements/movies-- movie reviews can be highly impacted by certain sequences in it, such reviews are often biased and do not provide a holistic feedback of the entire movie. Using our emotion recognition framework, one can evaluate movie sequences for distraction, for a better rating system and a feedback system for an immersive cinematic experience. Emotional human faces
(especially happy and anger) are ubiquitous on e-commerce websites specifically in categories like
clothing and accessories. These can act as stimuli to obtain EEG response and predict the gender 
to recommend appropriate products. As the window based analysis has shown, the stimulus time could 
be reduced to close to a second which is practically more feasible system so as to accelerate the GR
and provide a smooth customer experience. Furthermore, computers need to understand and adapt to user emotions for effective human-computer interaction, and gender-specific emotional aspects can be effectively utilized by affective interfaces for manipulating user behavior. 

%Overall, a number of correlations can be noted between explicit user responses, and their implicit brain activations during emotional face processing. Women recognized emotions, quicker and more correctly than men and correspondingly, better emotion recognition is achieved with female epochs. Women were especially sensitive to negative emotions, and this reflected in the form of stronger female ERP activations for negative emotions. 
 %
%obtained results confirm a strong correlation between  and their .  \textit{Fear} is the emotion least recognized at high and low intensity by male and female viewers, and it is also the worst recognized emotion from EEG brain signals in Fig.~\ref{Emrec}. \textit{Happy} is the emotion best recognized by viewers overall, and is well recognized along with \textit{disgust}, \textit{angry} and \textit{surprise} emotions from EEG responses. A discrepancy between RRs and EEG-based ER is however noted for the \textit{sad} emotion-- even though relatively high RRs are obtained for HI and LI \textit{sad} morphs, it is the second least recognized emotion after \textit{fear}. Overall, only slightly better-than-chance ER performance is achieved for all emotions with the two linear classifiers considered in this work. 
%
%Nevertheless, about 70\% gender recognition performance is achieved on comparing male and female EEG data specific to the six emotions. \textit{Anger} and \textit{disgust} are respectively the emotions for which gender-wise EEG signals can be best distinguished considering HI and LI morphs; maximum difference in male and female RRs is also noted for these emotions with HI and LI morphs. These findings suggest that emotional processing for these two emotions (and possibly, all negative emotions) happens differently for males and females. The obtained results reveal that it should be possible for user interfaces to recognize user gender anonymously, if users are willing to volunteer with the use of wearable sensors; this is a very plausible scenario if these sensors enhance user experience as with gaming.    
%This work examines gender-based differences in emotional face processing based on (i) explicit viewer recognition rates, and (ii) implicit EEG signals. The EEG signals enable recognition of viewer gender with around 70\% accuracy via simple linear classifiers. Future work will focus on (i) employing more sophisticated frameworks including deep neural networks, and (ii) examining other implicit behavioral signals for anonymous gender recognition. 
%
%
%All the more significant is the fact that the EEG signals are recorded via low-cost \textit{Emotiv} sensors, which have a relatively lower signal-to-noise ratio vis-\`a-vis lab devices, but can nevertheless be easily employed for large-scale user analytics.

 %Additionally, a significant difference is observed between males and females in fixation duration over eyes for mouth masked morphs which suggests females attend more to the eye region than males. While the previous works are skeptical about gender differences in the eye gaze, it is suggested that females often attend more to the eye regions than males while males attend more to the mouth than females .



==> data_analysis_backup.tex <==
\section{Materials and Methods}\label{MM}
%ACII_data_analysis
%This section details the experimental set-up and protocol used for our study.
Our study objective was to examine user behavior while viewing unoccluded/partly occluded emotional faces, and predict \emph{user gender} therefrom. We hypothesized that gender differences would be captured via EEG and eye-gaze patterns. Also, eye movements are known to be characteristic of the perceived facial emotion~\cite{schurgin}, which enables inference of the {stimulus emotion}; we limit ourselves to predicting the \emph{stimulus valence}, \ie, whether the face presented to the viewer exhibits a positive or negative emotion?

We designed a study to examine gender differences in visual emotional face processing with a) fully visible faces, and (b) faces with the \textit{eye} and \textit{mouth} regions occluded via a rectangular mask (Fig.~\ref{proto}). Salience of the occluded features towards conveying facial emotions is well known~\cite{subramanian2011can,schurgin}. Specifically, we considered emotional faces corresponding to four conditions: exhibiting \textit{high} intensity (\textbf{HI}) and \textit{low} intensity (\textbf{LI}) emotions, and additionally, \textit{high} intensity emotions upon occluding the \textit{eye} ({\textbf{eye-mask}}) or \textit{mouth} ({\textbf{mouth-mask}}) regions (Fig.~\ref{proto}). Since we hypothesized that emotion perception under facial occlusion would be considerably difficult (cf. Table~\ref{GenResults}), we did not study masked and mildly emotive faces. \\

\noindent \textbf{Participants:} 28 students from different nationalities (14 male, age $26.1\pm7.3$ and 14 female, age $25.5\pm6$), with normal or corrected vision, took part in our study. All users provided informed consent, and were presented a token fee for participation as directed by the ethics committee.  \\

\noindent \textbf{Stimuli:} We used emotional faces of 24 models (12 male, 12 female) from the {Radboud Faces Database} (RaFD)~\cite{Rafd}. RaFD includes facial emotions of 49 models rated for \textit{clarity}, \textit{genuineness} and \textit{intensity}, and the 24 models were chosen such that their Ekman facial emotions (\textbf{A}nger, \textbf{D}isgust, \textbf{F}ear, \textbf{H}appy, \textbf{Sa}d and \textbf{Su}rprise) were roughly matched based on these ratings. We then \textit{morphed} the emotive faces from \textit{neutral} (0\% intensity) to \textit{maximum} (100\% intensity) to generate intermediate morphs in steps of 5\%. Derived morphs with 55--100\% intensity were used as \textbf{HI} emotions, and 25--50\% were used as \textbf{LI} emotions. \textit{Eye} and \textit{mouth-masked} faces were automatically generated upon locating facial landmarks via Openface~\cite{Baltrusaitis2016} over the HI morphs. The \textit{eye mask} covered the eyes and nasion, while the \textit{mouth mask} covered the mouth and the nose ridge. All stimuli were resized to 361$\times$451 pixels, encompassing a visual angle of 9.1$^\circ$ and 11.4$^\circ$ about $x$ and $y$ at 60cm screen distance. \\

%\begin{figure}[!ht]
%    \centering
%\includegraphics[width=0.495\linewidth]{RT_M_vs_F_HI}\hspace{0.01in}\includegraphics[width=0.495\linewidth]{RT_M_vs_F_LI}
%\end{figure}
%
%%\begin{figure}[ht]
%%    \centering
%%\includegraphics[width=0.5\columnwidth]{RT_M_vs_F_LI}
%\caption{\label{RT_HR} Emotion-wise mean RTs of males and females considering HI(left) and LI(right) morphs. Error bars denote unit standard error (best-viewed in color).}
%\end{figure}
\noindent \textbf{Protocol:} The experimental protocol is outlined in Fig.\ref{proto}, and 
involved the presentation of \textit{unmasked} and \textit{masked} faces to viewers over two separate sessions, with a break in-between to avoid fatigue. We chose one face per model and emotion, resulting in 144 face images (1 morph/emotion $\times$ 6 emotions $\times$ 24 models). In the first session (\textit{no-mask} condition), these faces were shown in random order and were again re-presented randomly with an \textit{eye} or \textit{mouth mask} in the second session. We ensured a 50\% split of the HI and LI morphs in the first session, and eye/mouth-masked faces in the second.

During each trial, an emotional face was displayed for 4s preceded by a fixation cross for 500 ms. The viewer then had a maximum of 30s to make {one} out of {seven} choices concerning the facial emotion (six Ekman emotions plus neutral) via a radio button. Neutral faces were only utilized for morphing purposes and not used in the experiment. Viewers' EEG signals were acquired via the 14-channel \textit{Emotiv Epoc+} device, and eye movements were recorded with the \textit{Eyetribe} tracker during the trials. The face-viewing experiment was split into 4 segments to facilitate sensor re-calibration and minimize data recording errors, and took about 90 minutes to complete. 
\begin{figure*}[t]
	\includegraphics[width=0.95\linewidth]{Figures/protocol_newchanges.png} \vspace{-0.5cm}
   %\includegraphics[width=0.95\linewidth]{Figures/protocol_new2.png} {Protocol_new1.eps} \vspace{-0.4cm}
    \caption{\label{proto} \textbf{Experimental Protocol:} Viewers were required to recognize the facial emotion from either an \textit{unmasked} face (Session 1), or from an \textit{eye}/\textit{mouth} masked face (Session 2). Trial timelines for the two conditions are shown at the bottom.} \vspace{-0.5cm}
\end{figure*}

\section{User Responses}\label{DA}
We first compare male and female sensitivity to emotions based on \textit{explicitly} observed user response times (RTs) and recognition rates (RRs), and will then proceed to examine their \textit{implicit} eye movement and EEG responses. Our experimental design involved four \textit{stimulus types} (HI, LI, eye and mouth mask), and two \textit{user types} (male and female), resulting in $4 \times 2$ factor conditions.

% \subsection{No mask condition}
% \subsubsection{Response time (RT)}\label{RT_no}
% The overall viewer RT was 1.5$\pm$0.07 s, implying that users judged facial emotions fairly instantaneously. Table~\ref{tab:beh_stat} summarizes results from a 3-way ANOVA on RTs, with \textit{\textbf{morph intensity}} (MI) and \textit{facial \textbf{emotion}} as within-subject factors, and \textit{\textbf{gender}} as the between-subject factor. ANOVA revealed the main effect of MI with generally faster RTs noted for HI morphs (see Fig.~\ref{RT_HR}). The presented facial motion also impacted RTs, and pairwise comparisons revealed that RT for \textit{happy} ($1.3\pm0.9$ s) was significantly faster than for \textit{anger}, \textit{fear}, \textit{sad} and \textit{surprise}. ANOVA also revealed a marginal gender effect with females ($1.4\pm0.1$ s) generally responding faster than males ($1.6\pm0.1$ s). Significant interaction effects were also noted between (a) morph intensity and emotion, and (b) gender and emotion. %\textit{Angry} faces produced the highest RTs for males (mean RT = 1.9 s) while females took longest to judge \textit{surprise} (mean RT = 1.5 s). Conversely, lowest male RTs were noted for \textit{happy} (mean RT = 1.3 s), and lowest female RTs for \textit{disgust} (mean RT = 1.2 s). 
% As evident from Fig.~\ref{RT_HR}, females were significantly faster ($F(3,96)= 3.33, p < 0.05$) at judging negative (\textit{anger}, \textit{disgust}, \textit{fear} and \textit{sad}) emotions.

\begin{figure}[t]
%    \centering
\includegraphics[width=0.95\linewidth]{Figures/RTs-1_2_.png}%{ICMI_Figure_2.eps}
\caption{\label{RT_HR} \textbf{Emotion-wise RTs} of females and males in the various conditions. $y$-axis denotes response time in seconds. Error bars denote unit standard error (best-viewed in color).}
\vspace{-0.4cm}
\end{figure}

% \begin{table*}[ht!]
% \caption{ANOVA summary for behavioral measures. df and Sig respectively denote degrees of freedom and significance level.}\label{tab:beh_stat}\vspace{-.2cm}
% \centering
% \resizebox{0.75\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \toprule	
% \textbf{Response}	& \textbf{Predictor} & \multicolumn{1}{|p{0.25\columnwidth}|}{\centering{\textbf{Morph Intensity}}} & \textbf{Emotion} & \textbf{Gender} & \textbf{MI*Emotion}  &\textbf{ MI*Gender} & \textbf{Error} & \textbf{Total} \\ \toprule \bottomrule
% 	&\textbf{df} & 1 & 5 & 1 & 5 & 5 & 32 & 160 \\ 
% 	\multirow{ 2}{*}{\textbf{RT}} &\textbf{F} &  5.179 & 7.699 & 3.411 & 2.901 & 3.327 & & \\
% 	&\textbf{Sig} & $p<0.05$ & $p<0.001$ & $p = 0.074$ & $p<0.05$ & $p<0.05$ & & \\ 
% 	\multirow{ 2}{*}{\textbf{RR}} &\textbf{F} & 531.1 & 59.83  & 7.37  &  & 7.359 &  & \\
% 	&\textbf{Sig} & $p<0.001$ & $p<0.001$ & $p <0.05$ &  & $p<0.001$ &  & \\ \hline
% 	\end{tabular}}%\vspace{-.2cm}
% \end{table*}

% \subsubsection{Recognition rates (RRs)}\label{RR_no}
% A 64\% RR was achieved overall, suggesting that facial emotions were recognized well above chance level but well below ceiling. ANOVA summary in Table~\ref{tab:beh_stat} reveals the main effect of morph intensity, emotion and gender. Females were more accurate than males at recognizing negative emotions, even from LI morphs (Fig.~\ref{RRnfix}(a,b)). HI morphs were recognized more accurately (mean RR = 78.7) than LI morphs (mean RR = 49.1). Also, \textit{happy} faces were recognized most accurately, and \textit{fearful} faces least accurately.  We also found a significant interaction effect between morph intensity and emotion. Overall, (a) HI emotion morphs were recognized way more accurately than LI morphs, (b) females recognized negative emotions better than males and (c) \textit{Happy} was the easiest emotion to recognize, with \textit{fear} being the most difficult. 

\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{Figures/RRs-1_1_.png}%{ICMI_Figure_3.eps}
\caption{\label{RRnfix} \textbf{Emotion-wise RRs} in various conditions (view in color).} \vspace{-.5cm}
\end{figure}

%Two-sample $t$-tests showed that (i) females were significantly better at recognizing \textit{disgust} ($t(32)=3.14,p<0.05$), and (ii) HI \textit{angry} morphs were more accurately identified ($t(32)=-2.1081,p<0.05$) by females (M = 71\%) as compared to males (M = 57\%).
%
%\begin{marginfigure}[-20pc]
%  \begin{minipage}{\marginparwidth}
%    \centering
%    \includegraphics[width=\marginparwidth]{beh_HI} \centerline{(a)}\vspace{0.01cm}
%		\includegraphics[width=\marginparwidth]{beh_LI} \centerline{(b)}
%    \includegraphics[width=\marginparwidth]{Results_all_NB_HI} \centerline{(c)}\vspace{-.2cm}
%		%\includegraphics[width=\marginparwidth]{Results_all_LDA_LI} \centerline{(d)} \vspace{-.4cm}
%%\centerline{(a)\hspace{0.24\linewidth}(b)\hspace{0.24\linewidth}(c)\hspace{0.24\linewidth}(d)}
%\caption{\label{Emrec} Male (blue) and female (red) RRs for (a) HI morphs, and (b) LI morphs. (c) ER performance for \textit{all} HI epochs with NB classifier.  Error-bars denote unit standard deviation. View under zoom.} %* implies recognition is significantly higher than 0.5 ($p<0.05$), as given by a right-tailed $t$-test.}
%\end{minipage}
%\end{marginfigure}

%% edit begins

%% edit ends


\subsection{Response time (RT)}\label{RT_mask}
Overall user RTs for the HI, LI, {eye mask} and {mouth mask} conditions were respectively found to be 1.44 $\pm$ 0.24, 1.52 $\pm$ 0.05, 1.17 $\pm$ 0.12 and 1.25 $\pm$ 0.09 seconds, implying that FER was fairly instantaneous, and viewer responses were surprisingly faster with masked faces. Fine-grained comparison of male (\textit{m}) and female (\textit{f}) RTs across stimulus types (Fig.~\ref{RT_HR}) revealed that females ($\mu_{\text{RT}} = 1.40 \pm 0.10$s) were generally faster than males ($\mu_{\text{RT}} = 1.60 \pm 0.10$s) at recognizing {HI} emotions. There was no significant difference in RTs for {LI} emotions. Female alacrity nevertheless decreased for masked faces, with males responding marginally faster for \textit{eye masked} ($\mu_{\text{RT}}\text{(\textit{m})} = 1.13 \pm 0.11$s vs $\mu_{\text{RT}}\text{(\textit{f})} = 1.21 \pm 0.13$s), and both genders responding with similar speed for \textit{mouth masked} faces ($\mu_{\text{RT}}\text{(\textit{m})} = 1.24 \pm 0.10$s vs $\mu_{\text{RT}}\text{(\textit{f})} = 1.25 \pm 0.09$s). \\

%The mean response time observed during the emotional face processing is higher for males(1.6 $\pm$ 0.3) when compared to females(1.4 $\pm$ 0.1) under no mask condition however, this difference is insignificant for masked morphs. Despite happy being easily recognizable emotion for  all morph conditions, its RT is further lower for eye masked morphs than mouth masked ones. In addition, the difference between males and females in RT is insignificant for masked morphs when compared to no masked morphs indicating both the genders have encountered trouble in interpreting the emotion of the stimuli.
\subsection{Recognition Rates}\label{RR_mask}
While females recognized facial emotions marginally faster, we examined if they also achieved superior FER. Overall, RRs for unoccluded {HI} emotions ($\mu_{\text{RR}}=77.6$) were expectedly higher than for \textit{eye-masked} ($\mu_{\text{RR}}=59.7$), \textit{mouth-masked} ($\mu_{\text{RR}}=63.5$) and {LI} emotions ($\mu_{\text{RR}}=49.1$). Happy faces were recognized most accurately in all four conditions. Specifically focusing on gender differences (Fig.~\ref{RRnfix}), females recognized facial emotions more accurately than males and this was particularly true for \textit{negative} (A, D, F, S) emotions; male vs female RRs for these emotions differed significantly in the HI ($\mu_{\text{RR}}{(m)} =54.3$ vs $\mu_{\text{RR}} {(f)} =61.2, p<0.05$) and \textit{eye mask} conditions ($\mu_{\text{RR}}{(m)} =51.8$ vs $\mu_{\text{RR}}{(f)} =58.1, p<0.05$), and marginally for the \textit{mouth mask} condition 
($\mu_{\text{RR}}\text{(m)} =52$ vs $\mu_{\text{RR}} \text{(f)} =55.8, p=0.08$). Males marginally outperformed females in the  LI condition ($\mu_{\text{RR}}\text{(m)} = 49.8$ vs $\mu_{\text{RR}} \text{(f)} =47.7$). Overall, (a) HI emotion morphs were recognized more accurately than LI morphs, (b) females recognized negative emotions better, (c) \textit{Happy} was the easiest emotion to recognize, and (d) Higher RRs (across gender) were noted in the \emph{eye-mask} condition for four of the six Ekman emotions, implying that deformations around the mouth were more informative for FER under occlusion. 
% \begin{figure}[t]
% % \includegraphics[width = 0.49\linewidth]{RT_comp_lab}
% % \includegraphics[width = 0.49\linewidth]{RR_comp_lab}\vspace{-.1cm}
% \includegraphics[width = 1\linewidth]{ACII2017_Figure2.eps} \vspace{-0.3cm}
% \caption{ (a) RTs and (b) RRs for the three conditions. Error-bars denote unit standard error. View in color and under zoom.} \vspace{-0.5cm}
% \label{RTnRR}
% \end{figure}
%Anger and fear for mouth masked stimuli have shown on par RRs with no mask condition while it is significantly low for eye masked morphs. Happy (RR for no mask--97.5,upper half mask--97.8,lower half mask--84.4) remains most recognizable emotion for all three kinds of morphs. The RR for disgust and happy has dropped for mouth masked morphs.


%Participants were paid a token fee for their time and effort.

%The timing related specifics were same for the second session as the first, however instead of HI or LI morphed stimuli, the participants were shown upper or lower masked morphs of both HI and LI in random order. There were 4 parts of 72 trials each and had 288 face images presented per participant. They were asked to identify the emotion expressed by the stimuli based on the available information after masking.

%The experiment was conducted in a dimly lit room, and faces were displayed on a 14'' monitor placed 60 cm before the viewer. As participants viewed the faces and conveyed their judgments concerning the emotions, their eye movements were recorded using the \textit{Eyetribe} eye tracker. The Eyetribe has a sampling rate of 60 Hz and is accurate to within 0.5$^\circ$ visual angle upon calibration. To minimize tracking errors, both Ex 1 and Ex 2 were split into 4 parts, and the participant was allowed a break upon completion of each part. On resumption, the tracker was re-calibrated. A session comprising Ex 1 and Ex 2 typically took 90 minutes to complete, and participants were paid \$15 for their time.

%\subsection{Experiment 2}\label{MM}
%\textcolor {red} {\noindent \textbf{Occluded Information conditions}}\\
%
%\textcolor {red}{\noindent \textbf{Participants:} Same pool of participants from experiment 1 participated in this experiment. All participants gave informed consent and were paid for their participation.}
%
%\textcolor {red}{\noindent \textbf{Stimuli:} Stimuli used in this experiment were same as that used in experiment 1 with the difference being that all pictures either had a black box masking the mouth or eyes region. The masks at the eye or mouth region were counterbalanced and randomized across trials. }
%
%\textcolor {red}{\noindent \textbf{Protocol:} The experimental protocol was developed using Matlab\textsl{Psychtoolbox}~\cite{Psychtoolbox} and all conditions and experimental settings were similar to experiment 1. The experiment consisted of a total of 288 trials divided into 4 sessions of 72 images in each session. Eye-tracking data was recorded during the 4s duration when stimulus was displayed on the screen center during each trial. User response times and judgments about the emotion on the face image were also recorded.} 

\section{Analyzing Implicit Responses}\label{IC}
As females achieved quicker and superior FER for negative emotions, we hypothesized that these behavioral differences should also reflect via \emph{implicit} eye gaze and EEG patterns. We first describe the EEG and eye-movement descriptors employed for analyses, before discussing (stimulus) emotion and (user) gender recognition results.

\subsection{EEG preprocessing}\label{preprocessing}
We extracted EEG epochs for each trial (4.5s of stimulus-plus-fixation viewing time at 128 Hz sampling rate), and the 64 leading pre-stimulus samples were used to remove DC offset. This was followed by (a) EEG band-limiting to within 0.1--45 Hz, (b) Removal of noisy epochs via visual inspection, and (c) Independent component analysis (ICA) to remove artifacts relating to eye-blinks, and eye/muscle movements. Muscle movement artifacts in EEG are mainly concentrated in the 40--100 Hz band, and are removed upon band-limiting and via inspection of ICA components. Finally, a 7168 dimensional (14 channel $\times$4s$\times$128 Hz) EEG feature vector was generated and fed to different classifiers for GR and ER (Section~\ref{experiments}). 

\subsubsection{Event Related Potentials}\label{ERP}   
Event Related Potentials are time-locked neural responses related to sensory and cognitive events, and denote the EEG response averaged over multiple users and trials. As examples, P300 and N100, N400 are exemplar ERPs which are typically noted around 300, 100 and 400 ms post stimulus onset. ERPs occurring within 100 ms post stimulus onset are \emph{stimulus-related} (exogenous), while later ERPs are \emph{cognition-related} (endogenous). We examined the leading 128 EEG epoch samples (one second of data) for ERP patterns relating to emotion and gender. 

\begin{figure*}[t]
\includegraphics[width=0.48\linewidth]{Figures/ICMI_Figure_4a1.png}
\hspace{-1cm}
\includegraphics[width=0.48\linewidth]{Figures/ICMI_Figure_4a2.png}
\vspace{-2cm}
\includegraphics[width=0.48\linewidth]{Figures/ICMI_Figure_4b1.png}
\includegraphics[width=0.48\linewidth]{Figures/ICMI_Figure_4b2.png}
\vspace{1.4cm}
\caption{\label{ERP_HL} \textbf{ERPs} for {HI}  morphs (top) and {LI} morphs (bottom): (left to right) O1 and O2 ERPs for females and males. $y$-axis shows ERP amplitude in ${{\mu V}}$, refer (h) for legend. As per convention, ERPs are plotted upside down (view in color).} \vspace{-.4cm}
\end{figure*}

Prior works have observed ERP-based gender differences from lab-grade sensor recordings~\cite{Lithari2010,Muhl14,zotto2015processing}. Specifically,~\cite{Lithari2010} notes enhanced negative ERPs for females in response to negative valence stimuli. However, capturing ERPs with commercial devices is challenging due to their low signal-to-noise ratio~\cite{Vi2014}. Figs.~\ref{ERP_HL} and~\ref{ERPs1} present the P300, visual N100 and N400 ERP components in the occipital O1 and/or O2 electrodes (see Fig.~\ref{Emotiv} for sensor positions) corresponding to various face morphs. Note that the occipital lobe is the \textit{visual processing center} in the brain, as it contains the primary visual cortex. 

Comparing O1/O2 male and female ERPs for positive (H, Su) and negative (A, D, F, Sa) emotions, no significant differences can be observed between male positive and negative ERP peaks for HI or LI faces (columns 3,4 in Fig.\ref{ERP_HL}). However, we observe stronger N100 and P300 peaks in the negative female ERPs for both HI and LI faces (columns 1,2). Also, a stronger female N400 peak can be noted for HI faces consistent with prior findings~\cite{Lithari2010}. Contrastingly, lower male N100 and P300 latencies are observed for positive HI emotions, with the pattern being more obvious at O2. Likewise, lower male N400 latencies can be generally noted at O2 for positive emotions. The positive vs negative ERP difference for females is narrower for LI faces, revealing the difficulty in identifying mild LI emotions. That LI faces produce weaker ERPs at O1 and O2 than HI faces further supports this observation. 

Fig.~\ref{ERPs1} shows female ERPs observed in the occipital O2 electrode for the HI and \textit{eye mask} conditions. Clearly, one can note enhanced N100 and P300 ERP components for negative HI emotions (Fig.~\ref{ERPs1}(left)). This effect is attenuated in the \textit{eye mask} (Fig.~\ref{ERPs1}(right)) and \textit{mouth mask} cases, although one can note stronger N400 amplitudes for D and F with \textit{eye mask}. This ERP pattern is invisible for males, confirming thir gender-specificity. Overall, ERP patterns affirm that gender differences in emotional face processing can be reliably isolated with the low-cost \textit{Emotiv} device. 
\begin{figure}[t]
    \centering
%     \includegraphics[width=0.45\linewidth]{F-o2_HI_unmasked}\hspace{0.1cm}
%     \includegraphics[width=0.45\linewidth]{F-o2_eye_masked_erp}\vspace{-.1cm}
	  \includegraphics[width = 1.0\linewidth]{Figures/ACII2017_Figure3.png} \vspace{-0.3cm}
    \caption{\textbf{Female ERPs} in the (left) {HI}  and (right) {eye mask} conditions from the O2 channel. Best viewed in color.} \vspace{-0.5cm}
    \label{ERPs1}
\end{figure} 


%\begin{figure*}[ht]
    %
    %\includegraphics[width=0.245\textwidth]{M-o2_eye_masked_erp}
    %\includegraphics[width=0.245\textwidth]{F-o2_mouth_masked_erp}
    %\includegraphics[width=0.245\textwidth]{M-o2_mouth_masked_erp}
    %\caption{\label{ERPs2} \textbf{ERPs for masked stimuli:}  ERPs in males and females for eye masked and mouth masked morphs respectively in O2 region. Blue color represents positive emotions and red represents negative emotions. Best-viewed under zoom.}
%\end{figure*}

%While the presence of N100 and P300 are justified, since they have been observed previous \cite{Lithari2010}. In addition, we found N400 which in general is encountered for verbal stimuli in linguistics is also found for visual stimuli like photos and videos. The N400 for linguistic stimuli is found
%to emerge for conditions like shared representations and emotional valence. It also serves as an indicator for face recognition and examining object as well as actions and gesture processing\cite{kutas2011thirty}. In our case, since the task involves both facial processing and emotion recognition, its presence is strongly justified.
%
%It is evident from Figure-\ref{ERPs1} that the females have a stronger ERP components for negative emotions than positive emotions. Additionally, stronger N100 components are encountered for females than males which are in agreement with \cite{Lithari2010} at Pz electrode. The same scenario has been observed in O1 region as well.Also, lower N100 and P300 latencies can be observed for positive emotions in males.
%
%The N400 latency for positive emotions(happy, surprise) is lower than that of negative emotions for females when the upper half of face was masked however, when the lower half was masked, the difference in the latency is almost insignificant. For males, the latency of negative emotions is less than positive emotions for upper half masked morphs. The amplitude of N100 for negative emotions is greater in females than in males for masked morphs.

\subsection{Eye-tracking analysis}
Gender differences in gaze patterns during emotional face processing have been noted by prior works~\cite{schurgin,sullivan}. We used the low-cost \textit{Eyetribe} device with 30 Hz sampling to record eye movements. Raw gaze data output by the tracker were processed to compute \textit{fixations} (prolonged gazing at scene regions to assimilate visual information) and \emph{saccades} (transition from one fixation to another) via the EyeMMV toolbox~\cite{krassanakis2014eyemmv}. Upon extracting fixations and saccades, we extracted features employed for valence recognition in~\cite{Tavakoli15} to compute an 825-dimensional feature vector for our analyses.%, namely, saccade orientation, top-ten salient coordinates, saliency map and histograms of a) saccade slope, b) saccade length, c) saccade velocity, d) fixation duration, e) fixation count and f) saliency to compute an 825-dimensional feature vector for our analyses.   

%To compute  from  estimated by the tracker, we used the  and considered the  as a \textit{saccade}. 
\begin{figure*}[t]
\centering
% \includegraphics[width=0.24\linewidth]{Eye_fixation_dur_distr_unmask_ind}\hspace{0.1cm}
% \includegraphics[width=0.24\linewidth]{Eye_fixation_dur_distr_eyemask_ind}\hspace{0.1cm}\includegraphics[width=0.24\linewidth]{Eye_fixation_dur_distr_mouthmask_ind}\hspace{0.1cm}\includegraphics[width=0.24\linewidth]{valence_recogn_comp_lab}
\includegraphics[width = 0.95\linewidth]{Figures/fix_dur-1.png}%{ACII2017_Figure4.eps} \vspace{-0.3cm}
\caption{(a--d) \textbf{Fixation duration} distributions for males and females in the {HI}, {LI}, {eye} and {mouth-masked} conditions.}\vspace{-0.5cm}
\label{Fix_dur_dist}
\end{figure*}

\subsubsection{Fixation analysis}\label{Fix_anal}
To study gender differences in fixating patterns, we computed the distribution of fixation duration (FD) over six facial regions, namely, \textit{eyes}, \textit{nose}, \textit{mouth}, \textit{cheeks}, \textit{forehead} and \textit{chin}. Fig.~\ref{Fix_dur_dist} presents the males and female FD distribution over these facial regions for various conditions. For both genders, the time spent examining the eyes, nose and mouth accounted for over 80\% of the total FD, with eyes ($\approx$45\%) and nose ($\approx$30\%) attracting maximum attention as observed in \cite{schurgin,katti2010making,subramanian2011can}. Relatively similar FD distributions were noted for both genders with HI and LI morphs (Fig.~\ref{Fix_dur_dist} a,b). %However,  A decrease in the difference between males and females for LI morphs when compared to HI morphs in eye, mouth and forehead regions. The fixation duration in mouth region is slightly higher for LI morphs than HI. Females have marginally higher fixation duration for LI morphs in cheeks region than HI. %Focusing on the emotion-wise distributions, a high proportion of eye fixations is noted for all emotions except \textit{happy}, while relatively higher visual attention is noted on the nose and mouth for this emotion consistent with the findings in~\cite{schurgin} implying that these regions encode key emotional information concerning happiness. Overall, females were found to examine the eyes and mouth more for emotional cues, with males fixating more on the nose even though none of the differences were significant. The next section presents ER and GR results achieved with EEG and eye-based features. 

% \begin{figure}[t]
% %\includegraphics[width=0.49\linewidth]{Female_emotion_wise_fixation_dur_distr}\hspace{0.05cm}\includegraphics[width=0.49\linewidth]{Male_emotion_wise_fixation_dur_distr}\vspace{-.2cm}
% \centering
% \includegraphics[width=1.0\linewidth]{ICMI_Figure_5_1.eps}
% \vspace{-0.8cm}
% \caption{Fixation duration distributions: Region-wise fixation distribution across different emotions for (a) females and (b) males. Error bars denote unit standard error. \label{Fix_dist}}\vspace{-.2cm} 
% \end{figure}

Fig.\ref{Fix_dur_dist}(c,d) present FD distributions in the \textit{eye} and \textit{mouth mask} conditions. An independent $t$-test revealed a significant difference (\textit{p}$<$0.05) between male and female FDs for the eye region in the \textit{mouth mask} condition; prior works~\cite{wells2016identification} have observed that females primarily look at the eyes for emotional cues, which is mirrored by longer FDs around the eyes in the HI and \textit{mouth mask} conditions. Fig.\ref{Fix_dur_dist}(c) shows that when eye information is unavailable, females tend to focus on the mouth and nasal regions for FER.

\subsection{Experiments and Results}
\label{experiments}
Having noticed gender-specific patterns in user responses, EEG ERPs and eye movements, we attempted binary emotion recognition (ER) and gender recognition (GR) employing EEG features, eye-based features and their combination for the various conditions. {Recognition was attempted only on trials where viewers correctly recognized the presented facial emotion.}
We considered (i) EEG features, (ii) eye-based features, (iii) concatenation of the two (\textit{early fusion} or EF), and (iv) probabilistic fusion of the EEG and eye-based classifier outputs (\textit{late fusion} or LF) for our analyses. The $W_{est}$ technique~\cite{koelstra2012fusion} was used to fuse the EEG and eye-based outputs, and denotes \textit{maximum possible} recognition performance as optimal weights maximizing the test AUC metric were determined via a 2D grid search.

We considered the area under ROC curve ({\textbf{AUC}}) plotting true vs false positive rates, as the performance metric for benchmarking. AUC is suitable for evaluating classifier performance on unbalanced data, and a random classifier will achieve an AUC of 0.5.  As we attempted recognition with few training data, we report ER/GR results over five repetitions of 10-fold cross validation (CV) (\ie, total of 50 runs). CV is typically used to overcome the \textit{overfitting} problem, and train generalizable classifiers on small datasets. 

\subsubsection{Baseline Classification Approaches} 
As baselines, we considered the Naive-Bayes (NB), linear SVM (LSVM) and radial-basis SVM (RSVM) classifiers. NB is a generative classifier that estimates the test label based on the \emph{maximum a-posteriori} criterion,  $p(C\mid X)$, assuming class-conditional feature independence. $C$ and $X$ respectively denote test class-label and feature vector. LSVM and RSVM denote the linear and radial basis kernel versions of the Support Vector Machine (SVM) classifier. SVM hyperparameters $C$ (LSVM) and $\gamma$ (RSVM) were tuned from within $[10^{-4},10^{4}]$ via an inner 10-fold CV on the training set. 

%\subsubsection{Late Fusion} 
%For LF, we employed the $W_{est}$ technique~\cite{koelstra2012fusion} briefly described as follows. From the EEG and eye-based classifier outputs, the test set posterior probability for class $j$ is computed as $\sum_{i=1}^2 \alpha_i^*t_ip_i^j$, where $i$ indexes the two modalities, $p_i^j$'s denote posterior classifier probability for class  $j$ with modality $i$ and $\{\alpha_i^*\}$ are the optimal weights maximizing test performance, as determined via a 2D grid search. If $F_i$ denotes the training performance for the $i^{th}$ modality, then the normalized training performance $t_i = \alpha_i F_i/\sum_{i=1}^2 \alpha_i F_i$ for given $\alpha_i$. 

\subsubsection{CNN for EEG-based GR \& ER} 
Deep learning frameworks have recently become popular due to their ability to automatically learn optimal task features from raw data, thereby obviating the need for data cleaning and feature extraction. However, unlike in  image or video processing, temporal dynamics of the human brain are largely unclear; designing relevant features is therefore hard. We hypothesized that CNNs would encode EEG patterns efficiently, and also be robust to artifacts. These factors inspired us to feed \textit{raw} EEG data to a CNN, without any data processing (as in Sec.~\ref{preprocessing}); preprocessed EEG data was nevertheless fed to the above baseline classifiers.

%(in conclusion-add EEG data scarcity and explainability). 

\begin{figure*}
\vspace{0.05cm}
\centering
\includegraphics[width = 0.9\linewidth]{Figures/CNN_new.png}
\caption{\textbf{CNN architecture} showing various layers in the model and parameters.}\vspace{-0.5cm}
\label{DLarch}
\end{figure*}

We adopted a 3-layer Convolutional Neural Network (CNN)~\cite{MOHAMMADIANRAD2018180} to learn a robust EEG representation for gender and valence recognition. Three convolution layers together with rectified linear unit (ReLU) activation, and average pooling layers are stacked to learn EEG descriptors (Fig.~\ref{DLarch}). The convolutions employed are 1-dimensional along time. Batch normalization~\cite{pmlr-v37-ioffe15} is used after the third CNN layer to minimize covariate shift and accelerate training. To prevent overfitting, we used dropout after the fully connected layer with 128 neurons. A {softmax} over two output neurons was used for classification.

The number of kernels increase with network depth (cf. Fig~\ref{DLarch}) analogous to the VGG architecture~\cite{Simonyan14c}. We optimized the network for categorical cross-entropy loss using stochastic gradient descent with Nesterov momentum and weight decay. To decrease data dimensionality and avoid overfitting without sacrificing temporal EEG dependencies, we downsampled EEG data to 32Hz (reducing per-channel EEG dimensionality to 32$\times$4=128). A tenth of training data was used for validation and early-stopping enforced to prevent overfitting. CNN hyperparameters specified in Table~\ref{network_hyp} were either adopted from~\cite{MOHAMMADIANRAD2018180} or upon cross-validation. 

\input{network_table}

The CNN was traditionally trained for GR with \textit{He normal} initializers (normally distributed weights). Conversely, we adopted two-stage training for ER. In the first stage, the model was pre-trained with EEG data acquired over all four experimental conditions (Fig~\ref{proto}); the second stage involved fine-tuning with data for a specific condition. The objective here was to extract valence-related features irrespective of condition in the first stage, and fine-tune them to learn condition-specific descriptors. Experiments were designed using Keras~\cite{chollet2015keras} with Tensorflow back-end on a 16 GB CPU machine and an Intel i5 processor.
% Deep learning has been used succesfully used for several gaze based applications (cite Viral's HCII) however,
% 
\subsubsection{AdaBoost for ER from eye-gaze} %\textcolor{red}{(This section needs a serious revision!)}
% The gaze features as defined in section-\ref{preprocessing} consist of histograms of fixations, saccades and saliency based features. 
We employed the Adaboost classifier for ER from eye-gaze features. AdaBoost is an ensemble classifier popularly used for face detection~\cite{Viola:2004:RRF:966432.966458} and FER~\cite{silapachote2005feature}. Adaboost combines a number of weak classifiers (decision stumps), each marginally better than random, to cumulatively achieve optimal classification. The class label is based on the weighted output of each weak classifier. Our features (Sec.~\ref{preprocessing}) and classifier design were inspired by~\cite{silapachote2005feature}, who capture local dependencies via histograms of gaze measures like fixations, saccades and saliency. We employed SAMME (Stagewise Additive Modeling using a Multi-class Exponential loss function)~\cite{hastie2009multi} for training.  Similar to~\cite{silapachote2005feature}, local Gaussian and Gabor features were extracted at multiple scales to generate composite features for AdaBoost.  

We only obtained sparse gaze features in our study as viewer gaze was (a) localized to face regions of emotional importance and (b) recorded via a low-cost and low sampling rate device. We firstly performed feature selection to prune features relevant for ER. Feature selection was based on sequential addition (or removal) for optimal performance~\cite{Tavakoli15} using sequential forward (SFS) or backward (SBS) selection. The CNN and Adaboost models employed for GR and ER respectively are available at \url{https://github.com/bmaneesh/emotion-xavier}.
%To compare our results with the performance of classifiers like Naive-Bayes (NB), Linear Discriminant Analysis(LDA), linear SVM (LSVM) and radial-basis SVM (RSVM) classifiers\cite{maneesh2017icmi,maneesh2017acii}, we evaluate the classifiers for area under curve ({\textbf{AUC}}) measure. The reported results are based on the 10-fold cross validation. For both ER and GR, we only used (EEG and eye) data corresponding to \textit{correct} trials where users correctly recognized the presented facial emotion. 

\subsection{Results} \label{Results}
\subsubsection{Emotion Recognition} \label{ER}
We modeled stimulus ER as a binary classification problem, where the objective is to categorize \textit{positive} (H, Su) and \textit{negative} (A, D, F, Sa) valence stimuli employing gaze and EEG-based cues. ER results with (CNN-based) EEG, (Adaboost-based) eye gaze features, and late fusion of two modalities, with data acquired for different conditions characterized by user-gender (M/F) and stimulus type (HI/LI/eye-mask/mouth-mask) are shown in Fig.~\ref{Rec_Emotiv}. Evidently, gaze features perform significantly better than EEG. Gaze features achieve near-ceiling valence recognition barring the case where female users view LI emotions. Optimal performance is noted with male data for HI emotions (AUC = 0.99) similar to ~\cite{maneesh2017icmi}; ER from female eye-gaze data on HI emotions (AUC = 0.98) is also high.
 
On the other hand, ER results with EEG largely produced near-chance performance, with only male and female data for the {mouth-masked} condition being exceptions. These results reveal that the raw EEG features are not optimal for ER. Given the vast difference in ER performance with the gaze and EEG modalities, late fusion results are only occasionally superior to unimodal ones. Fusion slightly outperforms unimodal methods for the {eye mask} condition for both males (0.98 vs. 0.99) and females (0.97 vs. 0.98), and noticeably with males for {mouth mask} faces (0.91 vs. 0.94). 

%To summarize, gaze features outperform the EEG signals in ER during facial emotion recognition, EEG signals could give a reliable ER with \textit{mouth masked} morphs and probabilistic fusion of features is helpful for LI morphs with females and marginally helpful with other conditions. Emotional faces with partial information due to occlusion of mouth region provide better emotional cues than the ones with occlusion of eye region. The task of ER could be explored through emotional perception in addition to previous works like \cite{abadi2015decaf,Muhl14} that explicitly invoke emotions for the same.

%Fig.~\ref{Rec_Emotiv} presents valence recognition (VR) results obtained with male, female and male$+$female unimodal and multimodal features. Expectedly, better user-centered VR is achieved overall on examining responses to HI emotions (minimum AUC = 0.51 for HI vs 0.49 for LI morphs). Also, best VR performance is achieved with female data (mean AUC = 0.58 with HI morphs) as compared to male (mean AUC = 0.56, HI morphs) and male$+$female data (mean AUC = 0.543 for HI morphs) considering both unimodal and multimodal features. Interestingly, eye-based features (peak AUC = 0.64 with male data) are more discriminative for VR than EEG features (peak AUC = 0.53 with female data). Evidently, fusing the eye and EEG information is not beneficial even though a simple concatenation of the EEG and eye features is found to be superior to probabilistic fusion of unimodal results.

%Fig.\ref{Fix_dur_dist}(d) presents ER results obtained with the LDA classifier for male and female data, with unimodal and multimodal features for the three conditions. The best ER results are expectedly achieved for the no mask condition, and with eye-based features (AUC = 0.63 for females, and 0.64 for males), while minimal recognition is noted for the \textit{eye mask} condition reiterating the importance of eyes towards encoding emotional cues. EEG-based features only produce slightly better than chance recognition with a peak AUC score of 0.54. Multimodal recognition is slightly better than unimodal, and higher AUC scores are achieved in the masked conditions suggesting the complementarity of EEG and eye-based features when only partial facial information is available. 

\begin{figure}[t]
\includegraphics[width=0.95\linewidth]{Figures/val_dl.png}%{ICMI_Figure_6_1.eps}
%\includegraphics[width=0.48\linewidth,height=3cm]{fig_emotivpositions}
\vspace{-0.1cm}
\caption{\textbf{Valence recognition} results for different conditions.
} 
\label{Rec_Emotiv} \vspace{-.5cm} 
\end{figure}

%Our objective was not to induce emotions in viewers \textit{per se}-- the discriminability instead arises from the manner in which facial emotions are \textit{perceived} by viewers.
Overall, while recognizing the stimulus facial emotion was not our primary objective, the extracted gaze features are nevertheless highly effective for valence recognition.  Adaboost employing gaze features significantly outperforms the CNN trained with EEG data. The ability of eye movements to characterize emotional differences is unsurprising. Distinctive eye movement patterns have been observed while scanning scenes and faces with different emotions~\cite{schurgin,Subramanian2014,Tavakoli15}. Eye-based features are found to achieve 52.5\% VR accuracy in~\cite{Tavakoli15}, where emotions are induced by presenting diverse emotional scenes, while our study is specific to emotive faces. Prior neural studies~\cite{abadi2015decaf,Muhl14} which perform emotion recognition with lab-grade sensors achieve around 60\% VR. Superior performance of eye-based features can be attributed to the fact that the saccade and saliency-based statistics can capture discrepancies in gazing patterns for positive and negative facial emotions~\cite{Subramanian2014,Tavakoli15}; in contrast, neural features have only been moderately effective at decoding emotions conveyed by audio-visual music and movie stimuli~\cite{Koelstra2012,abadi2015decaf,Muhl14}, which can presumably elicit emotions more effectively than plain imagery.
 
\subsubsection{Gender Recognition}\label{GR_res}
GR involves labeling the test EEG or eye-gaze sample as arising from a \emph{male}/\emph{female} user. Table~\ref{tab:GenResults1} presents GR achieved with baseline classifiers, while Table~\ref{tab:GenResult2} shows AUC scores obtained with the EEG-based CNN, and the Adaboost ensemble fed with eye-gaze features. Both tables present GR results when user data corresponding to \textbf{All} emotional faces, and data for each of the six Ekman emotions (\textbf{Emotion-wise}) are employed for model training. Also, the best EF and LF results along with the relevant classifier are specified for the \textbf{All} condition. Cumulatively, Tables~\ref{tab:GenResults1} and~\ref{tab:GenResult2} clearly convey that the CNN and Adaboost frameworks considerably outperform baseline classifiers.

Focusing on Table~\ref{tab:GenResults1}, one can clearly note that the AUC scores with HI emotions are typically higher (cf. columns 1,2); also, AUC metrics achieved in the mouth-mask condition are typically higher than with eye-mask (columns 3,4). These findings from implicit user behavior mirror explicit recognition results in Fig.~\ref{RRnfix}. Specifically, significant differences can be noted with EEG-based results for the above conditions, while differences with eye-gaze are inconspicuous. These results cumulatively convey that (a) analyses of explicit and implicit user behavior affirm similar trends relating to visual FER; (b) gender differences are better encoded while perceiving high-intensity emotions, and how eye cues are interpreted for emotion inference, and (c) EEG signals better encode gender differences in visual emotion processing than gaze patterns.

Examining fusion results, LF is generally superior to EF when all emotions are considered, while EF achieves superior performance when emotion-specific user data are utilized for GR. We attempted GR from emotion-specific data to follow up on findings in Sec.~\ref{DA}, conveying females to be more sensitive to negative emotions. In Table~\ref{tab:GenResults1}, eye-gaze based GR performance improves significantly when emotion-specific data are considered (peak AUC of 0.68 for fear under eye-mask, vs peak AUC of 0.53 under mouth-mask for all emotions), while EEG results remain stable (peak AUC of 0.71 for HI anger vs peak AUC of 0.71 for all HI emotions). Optimal GR results (in bold) are mostly achieved for the A, D, F and Sa emotions implying that gender differences best manifest for negative valence.

Table~\ref{tab:GenResult2} largely replicates the trends noted from Table~\ref{tab:GenResults1}, with higher AUC scores achieved with the CNN and Adaboost classifiers. The one notable difference is that while the optimal NB baseline performs poorly with gaze features but much better with EEG in Table~\ref{tab:GenResults1}, the Adaboost framework outperforms the EEG-based CNN in the eye and mouth-mask conditions; EEG nevertheless encodes gender differences better while processing HI and LI emotions. These results imply that (a) eye movements in pursuit of FER, especially under partial face occlusion, are distinctive of gender, and (b) the discriminative Adaboost framework is able to better learn distinctive eye movement patterns as compared to the generative NB classifier. Late fusion results denoting the combination of decisions made by the CNN and Adaboost reveal that when one modality is considerably more potent than the other (EEG $>>$ Eye for HI and LI, while Eye $>$ EEG for mask), DF does not necessarily outperform constituent modalities.  

			%
%. While EEG performs better than gaze features for \textit{unmasked} morphs (HI-0.93 vs 0.52 and LI-0.88 vs 0.85), the gaze features significantly outperform EEG for \textit{masked} morphs (eye mask-0.97 vs 0.89 and mouth mask-0.97 vs 0.88). We believe that the better performance of gaze features over EEG is due to the significant difference between males and females as explained in sec-\ref{Fix_anal} for the masked conditions(in particular \textit{mouth mask} condition). Late fusion method performs close to the best modality for all morphs and better for \textit{eye mask} morphs. For emotion-wise GR with EEG, \textit{happy} morphs stimulate most differences in emotional perception between males and females however, it is to be noted that Sad and Happy perform closely. The emotion-wise comparison of EEG and gaze based GR confirms our previous observation of EEG outperforming gaze for HI and LI morphs but the inverse is true for \textit{masked} morphs. It is interesting to note that the GR is better for HI morphs than LI using EEG however, no such significant difference is observed with gaze. Gaze features reveals that \textit{anger} and \textit{sad} are the most discriminable emotions for \textit{unmasked} and \textit{masked} morphs respectively which is similar to our analysis with EEG where both \textit{anger} and \textit{sad} are close to \textit{happy}. 
%
%The late fusion strategy did not significantly improve the performance however, it outperformed the best of the either modalities for \textit{mouth mask} morphs for \textit{disgust} and \textit{surprise} emotions. Both EEG and late fusion strategy confirmed that LI morphs are least helpful in GR, masked morphs help in invoking better gender differences in emotional perception with \textit{mouth mask} morphs doing it the best. This has already been established through our initial evaluation of fixation duration (fig.\ref{Fix_dur_dist}(c)), we observe a significant difference between males and females for \textit{mouth mask} morphs.
%
%old stuff
%Table~\ref{GenResults} presents eye and EEG-based GR results obtained with HI and LI emotions. Specifically, GR AUC scores with various modalities and classifiers\footnote{with which optimal GR results are achieved for a given condition} corresponding to \textit{all} and \textit{emotion-specific} trials are tabulated. Clearly better than chance GR is achievable with both EEG and eye-based features. An immediate observation from the tabulated results is that unlike for ER, very similar GR performance is noted for both HI and LI emotions, implying that gender specific differences are also effectively encoded in implicit viewer responses to mildly emotive faces. This is consistent with the explicit user behavioral results in Fig.\ref{RRnfix}, where women are found to outperform men at recognizing LI facial emotions. 

\input{gender_all}
\input{gender_deep}

%Focusing on specifics, EEG features considerably outperform eye-based features for GR and higher AUC scores are obtained with \textit{emotion-specific} (exclusively negative emotion) features as compared to \textit{emotion agnostic} features. This finding is consistent with Fig.\ref{RRnfix} and prior works such as~\cite{Lithari2010,zotto2015processing} which have noted significant differences in female neural responses to negative facial emotions. Particularly, the best EEG AUC scores for HI and LI morphs are obtained for the anger and disgust emotions respectively, for which the greatest difference in recognition rates (of 0.14 and 0.13) can be observed from Fig.\ref{RRnfix}. These findings are salient and interesting, as Fig.\ref{RRnfix} and Table~\ref{GenResults} present two different phenomena, namely, gender differences in ER and discriminability of male and female EEG patterns.

%Surprisingly, multimodal fusion performs inferior to EEG/eye features. Also, marginally superior GR results are achieved with early fusion, suggesting that perhaps little complementary information is encoded between the EEG and eye-based features. Finally, RSVM is found to produce the best GR performance in most conditions implying that the extracted EEG and eye features are better separable in a higher-dimensional feature space. 

%\input{gender_mask}
%Table~\ref{GenResults} presents GR results with features extracted for (a) \textit{all} faces, and (b) \textit{emotion-specific} faces for the three conditions. The classifier employed for GR is also specified with parentheses. As with ER, the best GR performance (AUC = 0.71) is observed for the \textit{no mask} condition but with EEG features. With both EEG and eye-based cues, slightly higher GR performance is noted for the \textit{eye mask} condition as compared to the \textit{mouth mask} condition considering viewer responses for \textit{all} as well as \textit{emotion specific} faces. Overall, EEG features appear to encode gender differences better than eye-based features. Also, early or late fusion of the two modalities does not improve GR performance by much, even though one can note that fusion performs better than at least one of the modalities in the \textit{eye mask} and \textit{mouth mask} conditions. 

%A close examination of the emotion-wise results reveals that optimal GR is mainly achieved with viewer responses observed for negative facial emotions. This again is consistent with the observations from explicit user responses (Sec.\ref{DA}), where females were found to recognize negative facial emotions better than males. Overall, the obtained results point to systematic differences between males and females in the cognitive processing of emotional faces. Focusing on the standard deviation (sd) in AUC scores for emotion-wise GR, one can note much higher sd values in the \textit{eye mask} and \textit{mouth mask} conditions as compared to \textit{no mask}, indicating the difficulty in recognizing facial emotions under occlusion conditions. However, relatively lower sd values are noted with LF implying that probabilistic fusion enables better exploitation of the complementarity in the eye and brain-based signals, resulting in more robust GR. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%old ends

\subsubsection{Spatio-temporal EEG analysis} 
As EEG represents multi-channel time-series data, we also performed spatial and temporal analyses on the EEG signals to discover (i) the key EEG electrodes that capture gender differences in emotional face processing, and (ii) the critical time window for GR over the 4s (down-sampled) of stimulus presentation (or visual emotional processing).

A reliable GR was achieved for shorter time windows at various instants of stimuli presentation suggesting faster (less than 4s of stimuli presentation) GR possible and existence of gender differences throughout the stimuli duration (since the ERPs in sec.~\ref{ERP} only suggest gender differences in the first second from stimuli onset). Highest performance was observed with HI morphs while the least with \textit{eye mask} which is consistent with the trend in table-\ref{GenDeep}. The temporal analysis suggested no significant differences in GR among the windows however, best performance was observed for W-1,2 for all morph conditions suggesting early elicitation of differences in emotion processing consistent with our ERP analysis sec.\ref{ERP}. This difference is most observable for \textit{eye mask} and marginally for \textit{mouth mask} morphs (D,F,H,Sa). The masked morphs report higher standard deviation than full face morphs. This might be due to the difficulty induced due to occlusion of face regions in emotion recognition.

We evaluated each channel for their contribution to GR with the deep learning architecture configuration (fig.\ref{DLarch}) except with a slight modification of reducing the number of input channels to fit only one channel. The spatial analysis suggests possible GR with fewer channel devices that are available in market. Consistent with the findings in \cite{maneesh2017icmi,maneesh2017acii,Mclure04} we observed best performance with channels corresponding to Frontal and Occipital lobes of brain. The single electrode GR followed the trend as exhibited by table-\ref{GenDeep} \textit{i.e.,} HI, LI, \textit{eye mask} and \textit{mouth mask} morphs in descending order of GR. We observed a symmetric pattern among the best performing channels .i.e AF3 and AF4, and F3 and F4. While psychologists suggest the importance and utility for the brain hemispheres\cite{vingerhoets2003cerebral} in emotion recognition, its discussion deviates from the scope of our work.

%Fig.\ref{winGenResults}(a,b) show the temporal variance in GR performance for HI and LI morphs when the 4s emotional face viewing time is split into four 1s-long windows. These results are computed considering emotion-specific EEG epochs and with information from all 14 electrodes. Overall, no consistent temporal trends concerning gender discriminability can be noted from the plots. However, higher AUC scores over temporal windows  W1--W4 are achieved with LI morphs as compared to HI morphs. Also, slightly higher AUC metrics are noted for negative emotions especially with LI morphs, and the best and worst scores are obtained for the \textit{fear} and \textit{happy} emotions. Results of spatial analyses to identify the top three electrodes that best encode gender differences in emotion processing (EEG data over all 4s is used for this analysis.) are shown in Fig.\ref{winGenResults}(c). Again, superior GR is noted with LI morphs in this scenario, and five of the six electrodes with the best AUC scores correspond to the \textit{frontal} lobe. This result is consistent with the findings in ~\cite{Mclure04}, which notes that gender differences in emotion processing are best encoded in the prefrontal cortex. 

%Fig.\ref{winGRnVR}(a--c) show the temporal variance in GR performance for three considered conditions when the 4s presentation time is split into four 1s-long windows. These results are computed considering emotion-specific EEG epochs using RSVM. No significant difference in GR performance is observed over time for the \textit{no mask} scenario, and an AUC score of around 0.65 can be consistently noted over time. Barring exceptions, the GR AUC scores for the \textit{eye mask }and \textit{mouth mask} conditions are lower than for the \textit{no mask} condition. Also, maximum GR is predominantly noted for later temporal windows for mask conditions, implying that the discriminative cognitive processing between males and females happens later in time when only partial emotional information is made available to viewers. For the \textit{eye mask} scenario, maximum GR AUC scores are achieved for anger (AUC = 0.71 in W3), disgust (AUC = 0.65 in W1) and surprise (AUC = 0.65 in W2, W3 and W4). For the \textit{mouth mask} condition, highest AUCs are achieved for anger (AUC = 0.76 in W1 and 0.78 in W4), disgust (AUC = 0.68 in W2) and happy (AUC=0.69 in W2). However, low GR performance is generally noted over all time windows for the fear and surprise emotions in this condition, attributable to the general difficulty in recognizing these emotions when mouth-related information is unavailable. 

%Results of spatial analysis to identify the (top three) electrodes that best encode gender differences in emotion processing\footnote{EEG data over all 4s is used for this analysis.} are shown in Fig.\ref{winGRnVR}(d). In the \textit{no mask} condition, very similar AUC scores are observed for the frontal F8 (0.55), AF3 (0.52) and T7 (0.52) electrodes. Much higher numbers are noted for the \textit{eye mask} and \textit{mouth mask} conditions, suggesting that region-specific differences in cognitive processing for males and females manifest under occlusion conditions. For the \textit{eye mask} condition, highest AUCs are noted for O2 (0.87), P7 (0.81) and FC6 (0.76), while for \textit{mouth mask} F3 (AUC = 0.89), P7 (AUC = 0.87) and O1 (AUC = 0.87). An interesting observation is that a majority of the electrodes are located on the left hemisphere of the brain (see Emotiv electrode configuration for details).
%We observe from figure-\ref{winGRnVR}, that GR for masked morphs is better than no mask morphs in contrast, the performance of least performing electrodes has deteriorated for masked condition. The best performing electrode locations for no mask morphs are F8(0.55),T7 and AF4 while the least performing are F3,O2 and AF3(0.23). The best performing electrode locations for upper half mask morphs are O2(0.87),P7 and FC6 while the least performing are O1,FC5 and F7(0.03). The best performing electrode locations for lower half mask morphs are F3(0.89),P7 and O1 while the least performing are AF4,O2,FC5(0.06).
%
%From above results, it can be inferred that the best performing electrodes for no mask and upper half masked stimuli correspond to right hemisphere of brain and least performing electrodes to left hemisphere of the brain. The scenario is opposite for lower half masked stimuli. This is just a pattern we have observed and we have not encountered any literature that supports this statement.  

\begin{figure*}[th!]
\centering
\includegraphics[width=1.0\linewidth]{Figures/temporal_edited.png}%{Figures/temporal_new.jpg}%{ICMI_Figure_7_1.eps}
%\vspace{-0.7cm}
\caption{(a--d) \textbf{Temporal EEG analyses}: GR for {HI}, {LI}, {Eye} and {Mouth mask} conditions over temporal windows (W1--W4).} 
\label{winGenResults}
\vspace{-.4cm}
\end{figure*}


%}


%From figure- \ref{} GR based on time windows of 1 second of EEG responses give results significantly greater than chance level for both HI and LI morphs. \textit{fear} is the most discriminative emotion followed by \textit{anger} for both HI and LI morphs. The highest performance is observed irrespective of the emotions either for window-1 or window-4.

%\noindent \textbf{Main observations:} 

%This section examines the empirical results presented hitherto in the light of recent findings reported in literature. In particular, we consider the works of Schurgin \etal~\cite{schurgin}, Hall \etal~\cite{halljessica} and Sullivan \etal~\cite{sullivan}. Schurgin males may be sensitive to \etal~\cite{schurgin} observe that eye fixations mainly fall on the eyes, upper, lower nose and nasion and the upper lip while scanning emotional faces. Also, they note that different facial regions are focused on for each emotion, such as eyes for \textit{sad}, \textit{anger} and \textit{fear}, lips for \textit{happy} and upper lip for \textit{disgust} even though gender-based differences on visual attention are not analyzed. Hall \etal~and Sullivan \etal~expressly study gender differences while scanning emotional faces.  Hall \etal~\cite{halljessica} compute participant response times and recognition rates to conclude that women are faster and more accurate at emotion recognition, and solely attribute the enhanced emotion recognition capability of females to greater focusing on the eyes compared to males. Finally, Sullivan \etal~\cite{sullivan} observe that young and old women are superior to men at emotion recognition, and while women's looking at the eyes aids their facial emotion recognition, men's recognition rates correlate positively with their attention to the mouth.
%
%Our results mirror a number of these findings.\textcolor {red}{For both experiment 1 and 2 we found significant differences between morph and emotion types response times suggesting that certain morphs and emotions are overall faster as compared to others.For example we found that high-intensity Happy was the fastest and most accurately identified across all conditions. Fear had the lowest RR across all conditions.}
%
%\textcolor {red}{In Experiment 1 we see that overall, women took much less time than men to convey their emotional judgments and were also seen to be more accurate in identifying negative valence emotional images(Anger, Disgust, Fear and Sad) as compared to the positive valence face images (Happy and Surprise). The effects were more significant for the high-intensity images.} For low-intensity facial expressions, the overall emotion recognition performance for this condition was generally poor, with a large number of (mildly) expressive faces perceived as \textit{neutral}.\textcolor {red}{ We also find misperception between certain emotion types, for example, between \textit{anger}, \textit{disgust} and \textit{fear} and between \textit{surprise} and \textit{fear}.}
%
%\textcolor {red}{In Experiment 2 we found that to identify \textit{happy} emotion more information from mouth region is required to accurately recognize the emotion. \textit{Disgust} needed more of eye region information be correctly recognized. When the eye region is masked for both HI/LI morphs the RRs for males drop by approx 30\% and for females RRs drop by approx 40\% when compared to the no mask trials. This drop may be attributed to the fact that males concentrate more on the mouth region and females concentrate more on the eye regions and so when the eye region is masked female accuracy rates suffer more than their male counterparts.}
%
%Analysis of eye movement measures revealed that females attended more carefully to the expressive faces than men-- on average, they fixated more frequently and longer than males, while also making lengthier saccades. A fine-grained analysis of region-wise dwell times revealed that females attended more to the eyes across all emotions in the HI and LI conditions. On the other hand, men  are found to consistently fixate more on the cheek regions (discarded from analysis owing to negligible attention in~\cite{schurgin}). Men also attend more to the nose and mouth for at least two emotions in the HI and LI conditions. These fixation characteristics possibly explain their enhanced recognition of the LI \textit{disgust}, \textit{fear} and \textit{surprise} emotions over women.
%
%Some of the limitations of the presented study are (1) the analyzed recognition and eye movement-based statistics are compiled from a small subject population, and (ii) the use of a large number of \textit{low}-intensity expression morphs as stimuli (an equal number of HI and LI morphs were used), which were possibly difficult to recognize and therefore substantially perceived as \textit{neutral} by observers. Nevertheless, complementarity of the results observed from explicit viewer responses to the emotion recognition task, and implicit eye movements demonstrates the promise of the multimodal framework adopted for this study. 

%\textcolor{blue}{
%\section{Gaze analysis}
%Previous studies suggest the existence of differences in gaze patterns between males and females during emotional processing of faces\cite{schurgin} using traditional eye tracker devices with high sampling frequency. In this section, we evaluate the low-cost eye-tracker to validate its performance with respect to previous studies and also attempt to perform gender recognition using the same. The gaze response was collected at 30Hz sampling frequency. We have used \textit{fixation detection} from EyeMMV\cite{krassanakis2014eyemmv} package for extracting fixation information from the gaze responses. We have used the saccade orientation, histogram of saccade slope, histogram of saccade length,histogram of saccade velocity, histogram of fixation duration, fixation histogram, top-ten salient coordinates, saliency histogram and saliency map features as defined in \cite{Tavakoli15} to form a feature vector of 825 length. The samples are subjected to PCA dimensionality reduction to retain over 90\% variance for classification using NB, LDA and SVM. We employed \textit{Accuracy} and \textit{AUC} to evaluate the classifiers after 5 repetitions of 10 fold cross-validation.
%}

%\textcolor{blue}{
%\subsection{Eye-tracking analysis}
%In order to validate the tracker device, we have identified the distribution of fixations and fixation duration in six different face regions(forehead,eyes,nose,cheeks,mouth and chin). From the distribution of fixation duration across the face regions(refer \ref{fix_dur_HI}), it is clear that the time spent in the eyes,nose and mouth account for more than 80\% of the total time with eyes(45\%) and nose(30\%) attracting a major attention than mouth which is accordance with \cite{schurgin}.
%\begin{figure}
%\centering
%\includegraphics[width=0.25\textwidth]%{Eye_fixation_dur_distr_h}
%\caption{fixation duration histogram for HI}
%\label{fix_dur_HI}
%\end{figure}
%}

%\begin{figure}[ht]
%\centering
%\includegraphics[width=.3\textwidth]{valence_recogn_new}
%\caption{Valence recognition results over various modalities and %their fusions}
%\label{ValResults}
%\end{figure}

%\subsubsection{Valence Recognition}

%}

%\textcolor{blue}{
%From the valence recognition results figure-\ref{winGenResults} between positive and negative emotions, it is observed that the valence recognition for HI morphs is higher than LI morphs across the modalities confirming that the HI emotions are easily recognizable and more distinct when compared to the LI emotions. It is also to be noted that females perform better than males for both HI and LI morphs.
%}
%\textcolor{blue}{
%\begin{figure}[h]
%\centering\includegraphics[width=0.4\textwidth]{Results_all_NB_HI}
%\caption{ER performance for \textit{all} HI epochs with NB classifier}
%\label{Emrec}
%\end{figure}

 

%it is apparent since previous works reported a 60\% valence recognition using lab-grade sensors. The ER for masked stimuli is observed to be at chance level using EEG or eye tracking data but the fusion methods have achieved above chance results. It can observed that the performance for females is better than males for no mask and lower half masked morphs (strongly observable for early fusion). For upper half masked stimuli, though the difference between females and males is negligible, the early fusion results show that males are better at ER when lower part is visible, this can be justified from \cite{wells2016identification} that males attend more to mouth than females.


% \begin{figure*}
% \centering
% \includegraphics[width = 0.825\linewidth]{ACII2017_Figure5.eps} \vspace{-0.3cm}
% \caption{(a--c): Temporal variance in GR performance for the \textit{no mask}, \textit{eye mask} and \textit{mouth mask} conditions. (d) Top three electrodes showing best GR performance for the three conditions.}\vspace{-0.5cm}
% \label{winGRnVR}
% \end{figure*}
\input{temporal_dl.tex}

%Emotion wise GR using different modalities have been presented in table-\ref{GenResults} and it can observed that the GR using EEG responses out preform the other modalities. The highest GR is attained for anger and least for fear. This trend is consistent for masked morphs also. While Anger being most discriminative emotion between males and females, a significant performance drop can be noticed when upper half masked stimuli are presented over lower masked morphs. This is expected based on previous findings\cite{schurgin}. Fear is observed to perform better at discriminating genders with upper half masked morphs than lower half visible are presented. \textit{Schurgin et al} also observed that the recognition of happy was best for upper masked morphs, this is supported by a strong difference between GR using upper masked morphs and lower masked morphs by Early fusion and no significant differences were observed in GR for sad with either of the masks being used.


